Summarizing, Simplifying, and Synthesizing Medical Evidence Using GPT-3 (with Varying Success)

Large language models, particularly GPT-3, are able to produce high quality summaries of general domain news articles in few- and zero-shot settings. However, it is unclear if such models are similarly capable in more specialized, high-stakes domains such as biomedicine. In this paper, we enlist domain experts (individuals with medical training) to evaluate summaries of biomedical articles generated by GPT-3, given zero supervision. We consider both single- and multi-document settings. In the former, GPT-3 is tasked with generating regular and plain-language summaries of articles describing randomized controlled trials; in the latter, we assess the degree to which GPT-3 is able to \emph{synthesize} evidence reported across a collection of articles. We design an annotation scheme for evaluating model outputs, with an emphasis on assessing the factual accuracy of generated summaries. We find that while GPT-3 is able to summarize and simplify single biomedical articles faithfully, it struggles to provide accurate aggregations of findings over multiple documents. We release all data and annotations used in this work.

==> tables/multidoc_examples.tex <==
\begin{table*}[p]
    \small
    \centering
    \label{crouch}
    \begin{tabularx}{\textwidth}{X|p{3cm}|p{3cm}} \toprule
    \textbf{Input} & \textbf{Target} & \textbf{Generated} \\ \hline
        Study title: Felbamate add‐on therapy for drug‐resistant focal epilepsy
        \newline \newline
        Abstract title: Felbamate: a double-blind controlled trial in patients undergoing presurgical evaluation of partial seizures.
        \newline
        1. This double-blind, placebo-controlled trial studied the efficacy and safety of felbamate as an investigational antiepileptic drug. Sixty-four patients with refractory partial-onset seizures were given felbamate or placebo and monitored for time to fourth seizure. Results showed that felbamate was significantly better at reducing the occurrence of seizures compared to placebo (p = 0.028) and that adverse experiences with felbamate were generally mild or moderate in severity. This trial demonstrated that felbamate is an effective and safe treatment for refractory partial-onset seizures.
        \newline \newline
        Abstract title: Felbamate for partial seizures: results of a controlled clinical trial.
        \newline
        2. In a double-blind, placebo-controlled trial, 56 patients with partial seizures and a requirement for four or more seizures per month despite concomitant therapeutic blood levels of phenytoin and carbamazepine were given Felbamate. Results showed that Felbamate was statistically superior to the placebo in reducing seizures, with the mean seizure frequency for the 8-week trial period being 34.9 for Felbamate and 40.2 for placebo. Adverse experiences were minor, primarily consisting of nausea and CNS effects. Overall, this trial suggests that Felbamate is a safe and effective treatment for severely refractory epilepsy.
        \newline \newline
        Abstract title: Felbamate: a clinical trial for complex partial seizures.
        \newline
        3. This randomized, double-blind, three-period crossover study found that felbamate (FBM) was well-tolerated by 28 patients with complex partial seizures who continued taking carbamazepine (CBZ) throughout the trial. FBM was taken at a daily dose of 50 mg/kg (with a maximum of 3000 mg). There was a decrease in the CBZ levels during FBM periods (p less than 0.0001; 95\% confidence interval -28\%, -20\%). Although there was no significant reduction in seizure frequency between placebo and FBM periods, the data suggested a strong antiseizure effect of FBM when the lower CBZ levels were taken into account. 
        &
        In view of the methodological deficiencies, the limited number of included studies and the differences in outcome measures, we have found no reliable evidence to support the use of felbamate as an add-on therapy in people with drug-resistant focal-onset epilepsy. A large-scale, randomised controlled trial conducted over a longer period of time is required to inform clinical practice.
        &
        The evidence suggests that Felbamate is an effective and safe add-on therapy for patients with drug-resistant focal epilepsy. The trial showed that Felbamate was superior to placebo in reducing seizures, with no major adverse events reported. Additionally, the data suggests that Felbamate may have an antiseizure effect when combined with lower levels of carbamazepine.
    \end{tabularx}
    \caption{An example input for multi-document (regular) summarization}
\end{table*}


==> tables/singledoc_example_plain.tex <==
\begin{table*}[p]
    \small
    \centering
    \label{crouch}
    \begin{tabularx}{\textwidth}{X|p{3cm}|p{3cm}} \toprule
    \textbf{Input} & \textbf{Key results} & \textbf{Model Summary} \\ \hline
        OBJECT \newline
        We investigated the impact of a school-based 9-week mindfulness program vs. active control program (relaxation) and inactive control group on children's self-reported Health-Related Quality of Life (HRQoL) moderated by gender, grade, and independent practice.
        \newline \newline
        METHOD \newline
        In total 3519 (50/50\%  boys/girls) Finnish students aged 12-15 years from 56 schools were randomized into mindfulness intervention, active, and inactive control groups. HRQoL was measured at baseline, at 9 weeks, and at 26 weeks and analyzed with multilevel linear modeling.
        \newline \newline
        RESULTS \newline
        Significant improvement on HRQoL was found (β = mean difference) (β = 1.587, 95\% CI 0.672-2.502, p < 0.001) after 9 weeks and at 26 weeks of follow-up among students in the mindfulness group as compared to the active control group. Moderating effects on HRQoL were found for gender, grade, and independent practice: girls, 7th and 8th grade students, and students with regular independent mindfulness practice benefited most.
        \newline \newline
        CONCLUSIONS \newline
        Gender and developmental stage may moderate the effects of mindfulness interventions on HRQoL and offer guidance in designing effective promotive interventions for children and adolescents.
        \newline \newline
        TRIAL REGISTRATION INFORMATION \newline
        Healthy Learning Mind-a school-based mindfulness and relaxation program: a study protocol for a cluster randomized controlled trial (RCT) ISRCTN18642659 retrospectively registered on 13 October 2015. The full trial protocol can be accessed at http://rdcu.be/t57S .
        &
        RESULTS
        Significant improvement on HRQoL was found (β = mean difference) (β = 1.587, 95\%  CI 0.672-2.502, p < 0.001) after 9 weeks and at 26 weeks of follow-up among students in the mindfulness group as compared to the active control group.
        &
        This study investigated the impact of a 9-week school-based mindfulness program on Health-Related Quality of Life (HRQoL) in 3519 Finnish students aged 12-15, and found that girls, 7th and 8th grade students, and those with regular independent mindfulness practice benefited most. Moderating effects on HRQoL were found for gender, grade, and independent practice. The study protocol was retrospectively registered on 13 October 2015.
    \end{tabularx}
    \caption{An example input for single-document regular summarization}
\end{table*}


==> tables/singledoc_example_regular.tex <==
% \begin{table*}[p]
%     \small
%     \centering
%     \label{crouch}
%     \begin{tabularx}{\textwidth}{X|p{3cm}|p{3cm}|p{3cm}} \toprule
%     \textbf{Input} & \textbf{Key results} & \textbf{Model Summary} & \textbf{Simplified Model Summary} \\ \hline
%         OBJECT \newline
%         We investigated the impact of a school-based 9-week mindfulness program vs. active control program (relaxation) and inactive control group on children's self-reported Health-Related Quality of Life (HRQoL) moderated by gender, grade, and independent practice.
%         \newline \newline
%         METHOD \newline
%         In total 3519 (50/50\%  boys/girls) Finnish students aged 12-15 years from 56 schools were randomized into mindfulness intervention, active, and inactive control groups. HRQoL was measured at baseline, at 9 weeks, and at 26 weeks and analyzed with multilevel linear modeling.
%         \newline \newline
%         RESULTS \newline
%         Significant improvement on HRQoL was found (β = mean difference) (β = 1.587, 95\% CI 0.672-2.502, p < 0.001) after 9 weeks and at 26 weeks of follow-up among students in the mindfulness group as compared to the active control group. Moderating effects on HRQoL were found for gender, grade, and independent practice: girls, 7th and 8th grade students, and students with regular independent mindfulness practice benefited most.
%         \newline \newline
%         CONCLUSIONS \newline
%         Gender and developmental stage may moderate the effects of mindfulness interventions on HRQoL and offer guidance in designing effective promotive interventions for children and adolescents.
%         \newline \newline
%         TRIAL REGISTRATION INFORMATION \newline
%         Healthy Learning Mind-a school-based mindfulness and relaxation program: a study protocol for a cluster randomized controlled trial (RCT) ISRCTN18642659 retrospectively registered on 13 October 2015. The full trial protocol can be accessed at http://rdcu.be/t57S .
%         &
%         RESULTS
%         Significant improvement on HRQoL was found (β = mean difference) (β = 1.587, 95\%  CI 0.672-2.502, p < 0.001) after 9 weeks and at 26 weeks of follow-up among students in the mindfulness group as compared to the active control group.
%         &
%         This study investigated the impact of a 9-week school-based mindfulness program on Health-Related Quality of Life (HRQoL) in 3519 Finnish students aged 12-15, and found that girls, 7th and 8th grade students, and those with regular independent mindfulness practice benefited most. Moderating effects on HRQoL were found for gender, grade, and independent practice. The study protocol was retrospectively registered on 13 October 2015.
%         &
%         This study looked at whether a mindfulness program offered at school could help improve the quality of life of children aged 12-15. The study found that the mindfulness program did help, and that girls, 7th and 8th grade students, and students who practiced mindfulness on their own benefited the most. This means that gender and age can affect how helpful mindfulness programs are, and this information can help us design better programs for children and teenagers.
%     \end{tabularx}
%     \caption{An example input for single-document summarization (regular and simplified/plain)}
% \end{table*}

% REGULAR SINGLE DOC SUMMARIES
\begin{table*}[h]
    \small
    \centering
    \label{crouch}
    \begin{tabular}{l|l}
        \hline
        \textbf{Type of Error} & \textbf{Average Number of Summaries} \\ \hline
        \multicolumn{2}{l}{\textit{Population}} \\ \hline
        Omits demographic information & 1.33 \\
        Omits sample size & 36.33 \\
        Other & 1.0 \\ \hline
        \multicolumn{2}{l}{\textit{Intervention}} \\ \hline
        Does not describe comparator intervention & 5.33 \\
        Omits dosage or other important detail about administration & 4.33 \\
        Other & 1.67 \\ \hline
        \multicolumn{2}{l}{\textit{Outcome}} \\ \hline
        Omits description of specific measurements of high-level outcomes & 3 \\
        Omits one or more of multiple outcomes & 8 \\
        Other & 3.67 \\ \hline
    \end{tabular}
    \caption{Types of errors and the average number of articles for regular summarized documents}
\end{table*}

\begin{table*}[p]
    \small
    \centering
    \label{crouch}
    \begin{tabularx}{\textwidth}{X|p{3cm}|p{3cm}|p{3cm}} \toprule
    \textbf{Input} & \textbf{Key results} & \textbf{Model Summary} & \textbf{Simplified Model Summary} \\ \hline
        OBJECT \newline
        We investigated the impact of a school-based 9-week mindfulness program vs. active control program (relaxation) and inactive control group on children's self-reported Health-Related Quality of Life (HRQoL) moderated by gender, grade, and independent practice.
        \newline \newline
        METHOD \newline
        In total 3519 (50/50\%  boys/girls) Finnish students aged 12-15 years from 56 schools were randomized into mindfulness intervention, active, and inactive control groups. HRQoL was measured at baseline, at 9 weeks, and at 26 weeks and analyzed with multilevel linear modeling.
        \newline \newline
        RESULTS \newline
        Significant improvement on HRQoL was found (β = mean difference) (β = 1.587, 95\% CI 0.672-2.502, p < 0.001) after 9 weeks and at 26 weeks of follow-up among students in the mindfulness group as compared to the active control group. Moderating effects on HRQoL were found for gender, grade, and independent practice: girls, 7th and 8th grade students, and students with regular independent mindfulness practice benefited most.
        \newline \newline
        CONCLUSIONS \newline
        Gender and developmental stage may moderate the effects of mindfulness interventions on HRQoL and offer guidance in designing effective promotive interventions for children and adolescents.
        \newline \newline
        TRIAL REGISTRATION INFORMATION \newline
        Healthy Learning Mind-a school-based mindfulness and relaxation program: a study protocol for a cluster randomized controlled trial (RCT) ISRCTN18642659 retrospectively registered on 13 October 2015. The full trial protocol can be accessed at http://rdcu.be/t57S .
        &
        RESULTS
        Significant improvement on HRQoL was found (β = mean difference) (β = 1.587, 95\%  CI 0.672-2.502, p < 0.001) after 9 weeks and at 26 weeks of follow-up among students in the mindfulness group as compared to the active control group.
        &
        This study investigated the impact of a 9-week school-based mindfulness program on Health-Related Quality of Life (HRQoL) in 3519 Finnish students aged 12-15, and found that girls, 7th and 8th grade students, and those with regular independent mindfulness practice benefited most. Moderating effects on HRQoL were found for gender, grade, and independent practice. The study protocol was retrospectively registered on 13 October 2015.
        &
        This study looked at whether a mindfulness program offered at school could help improve the quality of life of children aged 12-15. The study found that the mindfulness program did help, and that girls, 7th and 8th grade students, and students who practiced mindfulness on their own benefited the most. This means that gender and age can affect how helpful mindfulness programs are, and this information can help us design better programs for children and teenagers.
    \end{tabularx}
    \caption{An example input for single-document summarization (regular and simplified/plain)}
\end{table*}


